Efficient Anytime CLF Reactive Planning System for a Bipedal Robot on Undulating Terrain

We propose and experimentally demonstrate a reactive planning system for bipedal robots on unexplored, challenging terrains. The system consists of a low-frequency planning thread (5 Hz) to find an asymptotically optimal path and a high-frequency reactive thread (300 Hz) to accommodate robot deviation. The planning thread includes: a multi-layer local map to compute traversability for the robot on the terrain; an anytime omnidirectional Control Lyapunov Function (CLF) for use with a Rapidly Exploring Random Tree Star (RRT*) that generates a vector field for specifying motion between nodes; a sub-goal finder when the final goal is outside of the current map; and a finite-state machine to handle high-level mission decisions. The system also includes a reactive thread to obviate the non-smooth motions that arise with traditional RRT* algorithms when performing path following. The reactive thread copes with robot deviation while eliminating non-smooth motions via a vector field (defined by a closed-loop feedback policy) that provides real-time control commands to the robot's gait controller as a function of instantaneous robot pose. The system is evaluated on various challenging outdoor terrains and cluttered indoor scenes in both simulation and experiment on Cassie Blue, a bipedal robot with 20 degrees of freedom. All implementations are coded in C++ with the Robot Operating System (ROS) and are available at https://github.com/UMich-BipedLab/CLF_reactive_planning_system.

==> ParameterStudy.tex <==

\section{Control Variables }
Fig.~\ref{fig:ControlParams}, we show how the control variables vary with
different start positions with a fixed orientation ($\theta=0$) and a fixed target
position $(\Gcal = (0, 0))$. In addition, we demonstrate how $\alpha$ in
\eqref{eq:optimization} affects control variables in
Fig.~\ref{fig:VariousAlphas}. One can observe that the larger $\alpha$ is, the larger
$v_y$ (the smaller $\omega$) would be. Therefore, $\alpha$ can be considered to represent the expense of lateral motion for the robot. Additionally, distance from the robot to
its goal affects the robot's behavior. 


\begin{figure*}[hb]
\centering
    \begin{subfigure}{0.64\columnwidth}
    \centering
    \label{fig:TrajVSAplha}%
\includegraphics[height=0.68\columnwidth]{AlphaVsTraj.png}~%
\caption{}
\end{subfigure}%
\begin{subfigure}{0.64\columnwidth}
    \centering
    \label{fig:TrajVSX}%
\includegraphics[height=0.68\columnwidth]{AlphaVsX.png}~
\caption{}
\end{subfigure}%
\begin{subfigure}{0.64\columnwidth}
    \centering
    \label{fig:TrajVSY}%
\includegraphics[height=0.68\columnwidth]{AlphaVsY.png}%
\caption{}
\end{subfigure}
\begin{subfigure}{0.64\columnwidth}
    \centering
    \label{fig:TrajVSTheta}
\includegraphics[height=0.68\columnwidth]{AlphaVsTheta.png}~
\caption{}
\end{subfigure}%
\begin{subfigure}{0.64\columnwidth}
    \centering
    \label{fig:TrajVSVx}%
\includegraphics[height=0.68\columnwidth]{AlphaVsVx.png}~%
\caption{}
\end{subfigure}%
\begin{subfigure}{0.64\columnwidth}
    \centering
    \label{fig:TrajVSVy}%
\includegraphics[height=0.68\columnwidth]{AlphaVsVy.png}
\caption{}
\end{subfigure}%
\caption[]{This figure demonstrates the resulting trajectories of different $\alpha$
values. The larger $\alpha$ is, the larger $v_y$ (the smaller $\omega$) would be; 
therefore, the change in $\theta$ is smaller.}%
\label{fig:VariousAlphas}%
\end{figure*}





\begin{figure*}[ht]
\centering
    \begin{subfigure}{0.65\columnwidth}
    \centering
\includegraphics[height=0.68\columnwidth]{ControlParams-vx.png}~%
\caption{}
    \label{fig:ControlVx}%
\end{subfigure}%
\begin{subfigure}{0.65\columnwidth}
    \centering
\includegraphics[height=0.68\columnwidth]{ControlParams-vy.png}~
\caption{}
    \label{fig:ControlVy}%
\end{subfigure}%
\begin{subfigure}{0.65\columnwidth}
    \centering
\includegraphics[height=0.68\columnwidth]{ControlParams-omega.png}
\caption{}
    \label{fig:ControlOmega}%
\end{subfigure}%
\caption[]{\add{Control parameters ($v_x, v_y, \omega$) given different start poses
    $(x, y, \theta=0)$ and a fixed target position $(0, 0)$.}
}
\label{fig:ControlParams}%
\end{figure*}
